Euclid. High signal-to-noise angular power spectrum reconstruction with limited sky coverage

We present NaturalSpice, a new Python implementation of the PolSpice angular power spectrum estimator. We show that the mixing matrix translating between pseudo and full-sky power spectra has eigenvalues given by the correlation function of the survey mask. Therefore, harmonic and real-space approaches to modelling mask effects are equivalent in the absence of a band limit. However, in real space the regularisation required for a given footprint can be consistently derived from its correlation function, which NaturalSpice employs by reformulating mode unmixing as a pseudo-inverse problem. We benchmark NaturalSpice against the widely used NaMaster algorithm using 200 fixed-cosmology light cone simulations applying three footprints representative of Euclid DR1 analyses (1600, 400, and 20 deg2). With a logistic apodisation function, NaturalSpice returns unbiased estimates with approximately 15, 30, and 60 per cent lower variance than NaMaster for the large, medium, and small footprints, respectively, and less correlated covariances for the two smaller footprints. These gains are concentrated at l < 100, while the two algorithms have equivalent performance on smaller scales. NaturalSpice is therefore particularly suited to early Stage-IV analyses with small-area but high-density datasets and as a tool to check for large-scale systematic effects. It is publicly available as part of the Euclid angular power spectra code Heracles

==> vlongauthor.tex <==
%%%% Version Wednesday 10th of December 2025 11:11:45 AM UT												
%%%% Please do not edit the author list -- contact ECEB Bureau for changes
\newcommand{\orcid}[1]{} %% if already defined in aa.cls: comment, or use renewcommand			   
\author{Euclid Collaboration: Y.~Fu\orcid{0000-0002-0759-0504}\thanks{\email{yfu@strw.leidenuniv.nl}}\inst{\ref{aff1},\ref{aff2}}
\and R.~Bouwens\orcid{0000-0002-4989-2471}\inst{\ref{aff1}}
\and K.~I.~Caputi\orcid{0000-0001-8183-1460}\inst{\ref{aff2},\ref{aff3}}
\and D.~Vergani\orcid{0000-0003-0898-2216}\inst{\ref{aff4}}
\and M.~Scialpi\orcid{0009-0006-5100-4986}\inst{\ref{aff5},\ref{aff6},\ref{aff7}}
\and B.~Margalef-Bentabol\orcid{0000-0001-8702-7019}\inst{\ref{aff8}}
\and L.~Wang\orcid{0000-0002-6736-9158}\inst{\ref{aff8},\ref{aff2}}
\and M.~Bolzonella\orcid{0000-0003-3278-4607}\inst{\ref{aff4}}
\and M.~Banerji\orcid{0000-0002-0639-5141}\inst{\ref{aff9}}
\and E.~Ba\~nados\orcid{0000-0002-2931-7824}\inst{\ref{aff10}}
\and A.~Feltre\orcid{0000-0001-6865-2871}\inst{\ref{aff7}}
\and Y.~Toba\orcid{0000-0002-3531-7863}\inst{\ref{aff11},\ref{aff12}}
\and J.~Calhau\orcid{0000-0003-1803-6899}\inst{\ref{aff13}}
\and F.~Tarsitano\orcid{0000-0002-5919-0238}\inst{\ref{aff14},\ref{aff15}}
\and P.~A.~C.~Cunha\orcid{0000-0002-9454-859X}\inst{\ref{aff16},\ref{aff17},\ref{aff18}}
\and A.~Humphrey\orcid{0000-0002-0510-2351}\inst{\ref{aff18},\ref{aff19}}
\and G.~Vietri\orcid{0000-0001-9155-8875}\inst{\ref{aff20}}
\and F.~Mannucci\orcid{0000-0002-4803-2381}\inst{\ref{aff7}}
\and S.~Bisogni\orcid{0000-0003-3746-4565}\inst{\ref{aff20}}
\and F.~Ricci\orcid{0000-0001-5742-5980}\inst{\ref{aff21},\ref{aff22}}
\and H.~Landt\orcid{0000-0001-8391-6900}\inst{\ref{aff23}}
\and L.~Spinoglio\orcid{0000-0001-8840-1551}\inst{\ref{aff24}}
\and T.~Matamoro~Zatarain\orcid{0009-0007-2976-293X}\inst{\ref{aff25}}
\and D.~Stern\orcid{0000-0003-2686-9241}\inst{\ref{aff26}}
\and M.~J.~Page\orcid{0000-0002-6689-6271}\inst{\ref{aff27}}
\and D.~M.~Alexander\orcid{0000-0002-5896-6313}\inst{\ref{aff23}}
\and G.~Zamorani\orcid{0000-0002-2318-301X}\inst{\ref{aff4}}
\and W.~Roster\orcid{0000-0002-9149-6528}\inst{\ref{aff28}}
\and M.~Salvato\orcid{0000-0001-7116-9303}\inst{\ref{aff28}}
\and Y.~Copin\orcid{0000-0002-5317-7518}\inst{\ref{aff29}}
\and J.~G.~Sorce\orcid{0000-0002-2307-2432}\inst{\ref{aff30},\ref{aff31}}
\and D.~Scott\orcid{0000-0002-6878-9840}\inst{\ref{aff32}}
\and Y.-H.~Zhang\orcid{0000-0003-4916-6346}\inst{\ref{aff1},\ref{aff33}}
\and E.~Lusso\orcid{0000-0003-0083-1157}\inst{\ref{aff5},\ref{aff7}}
\and J.~Wolf\orcid{0000-0003-0643-7935}\inst{\ref{aff10}}
\and D.~Yang\orcid{0000-0002-6769-0910}\inst{\ref{aff1}}
\and H.~J.~A.~Rottgering\orcid{0000-0001-8887-2257}\inst{\ref{aff1}}
\and B.~Laloux\orcid{0000-0001-9996-9732}\inst{\ref{aff13},\ref{aff28}}
\and M.~Siudek\orcid{0000-0002-2949-2155}\inst{\ref{aff34},\ref{aff35}}
\and S.~Belladitta\orcid{0000-0003-4747-4484}\inst{\ref{aff10},\ref{aff4}}
\and Q.~Liu\orcid{0000-0002-7490-5991}\inst{\ref{aff1}}
\and V.~Allevato\orcid{0000-0001-7232-5152}\inst{\ref{aff13}}
\and S.~Andreon\orcid{0000-0002-2041-8784}\inst{\ref{aff36}}
\and N.~Auricchio\orcid{0000-0003-4444-8651}\inst{\ref{aff4}}
\and C.~Baccigalupi\orcid{0000-0002-8211-1630}\inst{\ref{aff37},\ref{aff38},\ref{aff39},\ref{aff40}}
\and M.~Baldi\orcid{0000-0003-4145-1943}\inst{\ref{aff16},\ref{aff4},\ref{aff41}}
\and A.~Balestra\orcid{0000-0002-6967-261X}\inst{\ref{aff42}}
\and S.~Bardelli\orcid{0000-0002-8900-0298}\inst{\ref{aff4}}
\and P.~Battaglia\orcid{0000-0002-7337-5909}\inst{\ref{aff4}}
\and A.~Biviano\orcid{0000-0002-0857-0732}\inst{\ref{aff38},\ref{aff37}}
\and E.~Branchini\orcid{0000-0002-0808-6908}\inst{\ref{aff43},\ref{aff44},\ref{aff36}}
\and M.~Brescia\orcid{0000-0001-9506-5680}\inst{\ref{aff45},\ref{aff13}}
\and J.~Brinchmann\orcid{0000-0003-4359-8797}\inst{\ref{aff18},\ref{aff17},\ref{aff46}}
\and S.~Camera\orcid{0000-0003-3399-3574}\inst{\ref{aff47},\ref{aff48},\ref{aff49}}
\and G.~Ca\~nas-Herrera\orcid{0000-0003-2796-2149}\inst{\ref{aff50},\ref{aff1}}
\and V.~Capobianco\orcid{0000-0002-3309-7692}\inst{\ref{aff49}}
\and C.~Carbone\orcid{0000-0003-0125-3563}\inst{\ref{aff20}}
\and J.~Carretero\orcid{0000-0002-3130-0204}\inst{\ref{aff51},\ref{aff52}}
\and S.~Casas\orcid{0000-0002-4751-5138}\inst{\ref{aff53},\ref{aff54}}
\and M.~Castellano\orcid{0000-0001-9875-8263}\inst{\ref{aff22}}
\and G.~Castignani\orcid{0000-0001-6831-0687}\inst{\ref{aff4}}
\and S.~Cavuoti\orcid{0000-0002-3787-4196}\inst{\ref{aff13},\ref{aff55}}
\and K.~C.~Chambers\orcid{0000-0001-6965-7789}\inst{\ref{aff56}}
\and A.~Cimatti\inst{\ref{aff57}}
\and C.~Colodro-Conde\inst{\ref{aff58}}
\and G.~Congedo\orcid{0000-0003-2508-0046}\inst{\ref{aff33}}
\and C.~J.~Conselice\orcid{0000-0003-1949-7638}\inst{\ref{aff59}}
\and L.~Conversi\orcid{0000-0002-6710-8476}\inst{\ref{aff60},\ref{aff61}}
\and A.~Costille\inst{\ref{aff62}}
\and F.~Courbin\orcid{0000-0003-0758-6510}\inst{\ref{aff63},\ref{aff64}}
\and H.~M.~Courtois\orcid{0000-0003-0509-1776}\inst{\ref{aff65}}
\and M.~Cropper\orcid{0000-0003-4571-9468}\inst{\ref{aff27}}
\and A.~Da~Silva\orcid{0000-0002-6385-1609}\inst{\ref{aff66},\ref{aff67}}
\and H.~Degaudenzi\orcid{0000-0002-5887-6799}\inst{\ref{aff14}}
\and G.~De~Lucia\orcid{0000-0002-6220-9104}\inst{\ref{aff38}}
\and C.~Dolding\orcid{0009-0003-7199-6108}\inst{\ref{aff27}}
\and H.~Dole\orcid{0000-0002-9767-3839}\inst{\ref{aff31}}
\and F.~Dubath\orcid{0000-0002-6533-2810}\inst{\ref{aff14}}
\and C.~A.~J.~Duncan\orcid{0009-0003-3573-0791}\inst{\ref{aff33}}
\and X.~Dupac\inst{\ref{aff61}}
\and S.~Dusini\orcid{0000-0002-1128-0664}\inst{\ref{aff68}}
\and S.~Escoffier\orcid{0000-0002-2847-7498}\inst{\ref{aff69}}
\and M.~Fabricius\orcid{0000-0002-7025-6058}\inst{\ref{aff28},\ref{aff70}}
\and M.~Farina\orcid{0000-0002-3089-7846}\inst{\ref{aff24}}
\and R.~Farinelli\inst{\ref{aff4}}
\and S.~Ferriol\inst{\ref{aff29}}
\and F.~Finelli\orcid{0000-0002-6694-3269}\inst{\ref{aff4},\ref{aff71}}
\and P.~Fosalba\orcid{0000-0002-1510-5214}\inst{\ref{aff72},\ref{aff35}}
\and N.~Fourmanoit\orcid{0009-0005-6816-6925}\inst{\ref{aff69}}
\and M.~Frailis\orcid{0000-0002-7400-2135}\inst{\ref{aff38}}
\and E.~Franceschi\orcid{0000-0002-0585-6591}\inst{\ref{aff4}}
\and P.~Franzetti\inst{\ref{aff20}}
\and M.~Fumana\orcid{0000-0001-6787-5950}\inst{\ref{aff20}}
\and S.~Galeotta\orcid{0000-0002-3748-5115}\inst{\ref{aff38}}
\and K.~George\orcid{0000-0002-1734-8455}\inst{\ref{aff73}}
\and W.~Gillard\orcid{0000-0003-4744-9748}\inst{\ref{aff69}}
\and B.~Gillis\orcid{0000-0002-4478-1270}\inst{\ref{aff33}}
\and C.~Giocoli\orcid{0000-0002-9590-7961}\inst{\ref{aff4},\ref{aff41}}
\and J.~Gracia-Carpio\inst{\ref{aff28}}
\and A.~Grazian\orcid{0000-0002-5688-0663}\inst{\ref{aff42}}
\and F.~Grupp\inst{\ref{aff28},\ref{aff70}}
\and L.~Guzzo\orcid{0000-0001-8264-5192}\inst{\ref{aff74},\ref{aff36},\ref{aff75}}
\and S.~V.~H.~Haugan\orcid{0000-0001-9648-7260}\inst{\ref{aff76}}
\and H.~Hoekstra\orcid{0000-0002-0641-3231}\inst{\ref{aff1}}
\and W.~Holmes\inst{\ref{aff26}}
\and I.~M.~Hook\orcid{0000-0002-2960-978X}\inst{\ref{aff77}}
\and F.~Hormuth\inst{\ref{aff78}}
\and A.~Hornstrup\orcid{0000-0002-3363-0936}\inst{\ref{aff79},\ref{aff80}}
\and K.~Jahnke\orcid{0000-0003-3804-2137}\inst{\ref{aff10}}
\and M.~Jhabvala\inst{\ref{aff81}}
\and B.~Joachimi\orcid{0000-0001-7494-1303}\inst{\ref{aff82}}
\and E.~Keih\"anen\orcid{0000-0003-1804-7715}\inst{\ref{aff83}}
\and S.~Kermiche\orcid{0000-0002-0302-5735}\inst{\ref{aff69}}
\and A.~Kiessling\orcid{0000-0002-2590-1273}\inst{\ref{aff26}}
\and B.~Kubik\orcid{0009-0006-5823-4880}\inst{\ref{aff29}}
\and M.~K\"ummel\orcid{0000-0003-2791-2117}\inst{\ref{aff70}}
\and M.~Kunz\orcid{0000-0002-3052-7394}\inst{\ref{aff84}}
\and H.~Kurki-Suonio\orcid{0000-0002-4618-3063}\inst{\ref{aff85},\ref{aff86}}
\and R.~Laureijs\inst{\ref{aff2}}
\and A.~M.~C.~Le~Brun\orcid{0000-0002-0936-4594}\inst{\ref{aff87}}
\and S.~Ligori\orcid{0000-0003-4172-4606}\inst{\ref{aff49}}
\and P.~B.~Lilje\orcid{0000-0003-4324-7794}\inst{\ref{aff76}}
\and V.~Lindholm\orcid{0000-0003-2317-5471}\inst{\ref{aff85},\ref{aff86}}
\and I.~Lloro\orcid{0000-0001-5966-1434}\inst{\ref{aff88}}
\and G.~Mainetti\orcid{0000-0003-2384-2377}\inst{\ref{aff89}}
\and D.~Maino\inst{\ref{aff74},\ref{aff20},\ref{aff75}}
\and E.~Maiorano\orcid{0000-0003-2593-4355}\inst{\ref{aff4}}
\and O.~Mansutti\orcid{0000-0001-5758-4658}\inst{\ref{aff38}}
\and S.~Marcin\inst{\ref{aff90}}
\and O.~Marggraf\orcid{0000-0001-7242-3852}\inst{\ref{aff91}}
\and K.~Markovic\orcid{0000-0001-6764-073X}\inst{\ref{aff26}}
\and M.~Martinelli\orcid{0000-0002-6943-7732}\inst{\ref{aff22},\ref{aff92}}
\and N.~Martinet\orcid{0000-0003-2786-7790}\inst{\ref{aff62}}
\and F.~Marulli\orcid{0000-0002-8850-0303}\inst{\ref{aff93},\ref{aff4},\ref{aff41}}
\and R.~J.~Massey\orcid{0000-0002-6085-3780}\inst{\ref{aff94}}
\and E.~Medinaceli\orcid{0000-0002-4040-7783}\inst{\ref{aff4}}
\and S.~Mei\orcid{0000-0002-2849-559X}\inst{\ref{aff95},\ref{aff96}}
\and M.~Melchior\inst{\ref{aff97}}
\and Y.~Mellier\inst{\ref{aff98},\ref{aff99}}
\and M.~Meneghetti\orcid{0000-0003-1225-7084}\inst{\ref{aff4},\ref{aff41}}
\and E.~Merlin\orcid{0000-0001-6870-8900}\inst{\ref{aff22}}
\and G.~Meylan\inst{\ref{aff100}}
\and A.~Mora\orcid{0000-0002-1922-8529}\inst{\ref{aff101}}
\and M.~Moresco\orcid{0000-0002-7616-7136}\inst{\ref{aff93},\ref{aff4}}
\and L.~Moscardini\orcid{0000-0002-3473-6716}\inst{\ref{aff93},\ref{aff4},\ref{aff41}}
\and R.~Nakajima\orcid{0009-0009-1213-7040}\inst{\ref{aff91}}
\and C.~Neissner\orcid{0000-0001-8524-4968}\inst{\ref{aff102},\ref{aff52}}
\and R.~C.~Nichol\orcid{0000-0003-0939-6518}\inst{\ref{aff103}}
\and S.-M.~Niemi\orcid{0009-0005-0247-0086}\inst{\ref{aff50}}
\and C.~Padilla\orcid{0000-0001-7951-0166}\inst{\ref{aff102}}
\and S.~Paltani\orcid{0000-0002-8108-9179}\inst{\ref{aff14}}
\and F.~Pasian\orcid{0000-0002-4869-3227}\inst{\ref{aff38}}
\and K.~Pedersen\inst{\ref{aff104}}
\and W.~J.~Percival\orcid{0000-0002-0644-5727}\inst{\ref{aff105},\ref{aff106},\ref{aff107}}
\and V.~Pettorino\orcid{0000-0002-4203-9320}\inst{\ref{aff50}}
\and S.~Pires\orcid{0000-0002-0249-2104}\inst{\ref{aff108}}
\and G.~Polenta\orcid{0000-0003-4067-9196}\inst{\ref{aff109}}
\and M.~Poncet\inst{\ref{aff110}}
\and L.~A.~Popa\inst{\ref{aff111}}
\and L.~Pozzetti\orcid{0000-0001-7085-0412}\inst{\ref{aff4}}
\and F.~Raison\orcid{0000-0002-7819-6918}\inst{\ref{aff28}}
\and R.~Rebolo\orcid{0000-0003-3767-7085}\inst{\ref{aff58},\ref{aff112},\ref{aff113}}
\and A.~Renzi\orcid{0000-0001-9856-1970}\inst{\ref{aff114},\ref{aff68}}
\and J.~Rhodes\orcid{0000-0002-4485-8549}\inst{\ref{aff26}}
\and G.~Riccio\inst{\ref{aff13}}
\and E.~Romelli\orcid{0000-0003-3069-9222}\inst{\ref{aff38}}
\and M.~Roncarelli\orcid{0000-0001-9587-7822}\inst{\ref{aff4}}
\and E.~Rossetti\orcid{0000-0003-0238-4047}\inst{\ref{aff16}}
\and R.~Saglia\orcid{0000-0003-0378-7032}\inst{\ref{aff70},\ref{aff28}}
\and Z.~Sakr\orcid{0000-0002-4823-3757}\inst{\ref{aff115},\ref{aff116},\ref{aff117}}
\and D.~Sapone\orcid{0000-0001-7089-4503}\inst{\ref{aff118}}
\and B.~Sartoris\orcid{0000-0003-1337-5269}\inst{\ref{aff70},\ref{aff38}}
\and M.~Schirmer\orcid{0000-0003-2568-9994}\inst{\ref{aff10}}
\and P.~Schneider\orcid{0000-0001-8561-2679}\inst{\ref{aff91}}
\and T.~Schrabback\orcid{0000-0002-6987-7834}\inst{\ref{aff119}}
\and M.~Scodeggio\inst{\ref{aff20}}
\and A.~Secroun\orcid{0000-0003-0505-3710}\inst{\ref{aff69}}
\and E.~Sefusatti\orcid{0000-0003-0473-1567}\inst{\ref{aff38},\ref{aff37},\ref{aff39}}
\and G.~Seidel\orcid{0000-0003-2907-353X}\inst{\ref{aff10}}
\and S.~Serrano\orcid{0000-0002-0211-2861}\inst{\ref{aff72},\ref{aff120},\ref{aff35}}
\and P.~Simon\inst{\ref{aff91}}
\and C.~Sirignano\orcid{0000-0002-0995-7146}\inst{\ref{aff114},\ref{aff68}}
\and G.~Sirri\orcid{0000-0003-2626-2853}\inst{\ref{aff41}}
\and L.~Stanco\orcid{0000-0002-9706-5104}\inst{\ref{aff68}}
\and J.-L.~Starck\orcid{0000-0003-2177-7794}\inst{\ref{aff108}}
\and J.~Steinwagner\orcid{0000-0001-7443-1047}\inst{\ref{aff28}}
\and C.~Surace\orcid{0000-0003-2592-0113}\inst{\ref{aff62}}
\and P.~Tallada-Cresp\'{i}\orcid{0000-0002-1336-8328}\inst{\ref{aff51},\ref{aff52}}
\and D.~Tavagnacco\orcid{0000-0001-7475-9894}\inst{\ref{aff38}}
\and A.~N.~Taylor\inst{\ref{aff33}}
\and H.~I.~Teplitz\orcid{0000-0002-7064-5424}\inst{\ref{aff121}}
\and I.~Tereno\orcid{0000-0002-4537-6218}\inst{\ref{aff66},\ref{aff122}}
\and N.~Tessore\orcid{0000-0002-9696-7931}\inst{\ref{aff82}}
\and S.~Toft\orcid{0000-0003-3631-7176}\inst{\ref{aff3},\ref{aff123}}
\and R.~Toledo-Moreo\orcid{0000-0002-2997-4859}\inst{\ref{aff124}}
\and F.~Torradeflot\orcid{0000-0003-1160-1517}\inst{\ref{aff52},\ref{aff51}}
\and I.~Tutusaus\orcid{0000-0002-3199-0399}\inst{\ref{aff35},\ref{aff72},\ref{aff116}}
\and L.~Valenziano\orcid{0000-0002-1170-0104}\inst{\ref{aff4},\ref{aff71}}
\and J.~Valiviita\orcid{0000-0001-6225-3693}\inst{\ref{aff85},\ref{aff86}}
\and T.~Vassallo\orcid{0000-0001-6512-6358}\inst{\ref{aff38}}
\and A.~Veropalumbo\orcid{0000-0003-2387-1194}\inst{\ref{aff36},\ref{aff44},\ref{aff43}}
\and D.~Vibert\orcid{0009-0008-0607-631X}\inst{\ref{aff62}}
\and Y.~Wang\orcid{0000-0002-4749-2984}\inst{\ref{aff121}}
\and J.~Weller\orcid{0000-0002-8282-2010}\inst{\ref{aff70},\ref{aff28}}
\and A.~Zacchei\orcid{0000-0003-0396-1192}\inst{\ref{aff38},\ref{aff37}}
\and E.~Zucca\orcid{0000-0002-5845-8132}\inst{\ref{aff4}}
\and M.~Ballardini\orcid{0000-0003-4481-3559}\inst{\ref{aff125},\ref{aff126},\ref{aff4}}
\and E.~Bozzo\orcid{0000-0002-8201-1525}\inst{\ref{aff14}}
\and C.~Burigana\orcid{0000-0002-3005-5796}\inst{\ref{aff127},\ref{aff71}}
\and R.~Cabanac\orcid{0000-0001-6679-2600}\inst{\ref{aff116}}
\and M.~Calabrese\orcid{0000-0002-2637-2422}\inst{\ref{aff128},\ref{aff20}}
\and A.~Cappi\inst{\ref{aff4},\ref{aff129}}
\and D.~Di~Ferdinando\inst{\ref{aff41}}
\and J.~A.~Escartin~Vigo\inst{\ref{aff28}}
\and L.~Gabarra\orcid{0000-0002-8486-8856}\inst{\ref{aff130}}
\and W.~G.~Hartley\inst{\ref{aff14}}
\and M.~Huertas-Company\orcid{0000-0002-1416-8483}\inst{\ref{aff58},\ref{aff34},\ref{aff131},\ref{aff132}}
\and J.~Mart\'{i}n-Fleitas\orcid{0000-0002-8594-569X}\inst{\ref{aff133}}
\and S.~Matthew\orcid{0000-0001-8448-1697}\inst{\ref{aff33}}
\and N.~Mauri\orcid{0000-0001-8196-1548}\inst{\ref{aff57},\ref{aff41}}
\and R.~B.~Metcalf\orcid{0000-0003-3167-2574}\inst{\ref{aff93},\ref{aff4}}
\and A.~A.~Nucita\inst{\ref{aff134},\ref{aff135},\ref{aff136}}
\and A.~Pezzotta\orcid{0000-0003-0726-2268}\inst{\ref{aff36}}
\and M.~P\"ontinen\orcid{0000-0001-5442-2530}\inst{\ref{aff85}}
\and C.~Porciani\orcid{0000-0002-7797-2508}\inst{\ref{aff91}}
\and I.~Risso\orcid{0000-0003-2525-7761}\inst{\ref{aff36},\ref{aff44}}
\and V.~Scottez\orcid{0009-0008-3864-940X}\inst{\ref{aff98},\ref{aff137}}
\and M.~Sereno\orcid{0000-0003-0302-0325}\inst{\ref{aff4},\ref{aff41}}
\and M.~Tenti\orcid{0000-0002-4254-5901}\inst{\ref{aff41}}
\and M.~Viel\orcid{0000-0002-2642-5707}\inst{\ref{aff37},\ref{aff38},\ref{aff40},\ref{aff39},\ref{aff138}}
\and M.~Wiesmann\orcid{0009-0000-8199-5860}\inst{\ref{aff76}}
\and Y.~Akrami\orcid{0000-0002-2407-7956}\inst{\ref{aff139},\ref{aff140}}
\and S.~Alvi\orcid{0000-0001-5779-8568}\inst{\ref{aff125}}
\and I.~T.~Andika\orcid{0000-0001-6102-9526}\inst{\ref{aff141},\ref{aff142}}
\and S.~Anselmi\orcid{0000-0002-3579-9583}\inst{\ref{aff68},\ref{aff114},\ref{aff143}}
\and M.~Archidiacono\orcid{0000-0003-4952-9012}\inst{\ref{aff74},\ref{aff75}}
\and F.~Atrio-Barandela\orcid{0000-0002-2130-2513}\inst{\ref{aff144}}
\and E.~Aubourg\orcid{0000-0002-5592-023X}\inst{\ref{aff95},\ref{aff145}}
\and D.~Bertacca\orcid{0000-0002-2490-7139}\inst{\ref{aff114},\ref{aff42},\ref{aff68}}
\and M.~Bethermin\orcid{0000-0002-3915-2015}\inst{\ref{aff146}}
\and L.~Bisigello\orcid{0000-0003-0492-4924}\inst{\ref{aff42}}
\and A.~Blanchard\orcid{0000-0001-8555-9003}\inst{\ref{aff116}}
\and L.~Blot\orcid{0000-0002-9622-7167}\inst{\ref{aff147},\ref{aff87}}
\and M.~Bonici\orcid{0000-0002-8430-126X}\inst{\ref{aff105},\ref{aff20}}
\and S.~Borgani\orcid{0000-0001-6151-6439}\inst{\ref{aff148},\ref{aff37},\ref{aff38},\ref{aff39},\ref{aff138}}
\and M.~L.~Brown\orcid{0000-0002-0370-8077}\inst{\ref{aff59}}
\and S.~Bruton\orcid{0000-0002-6503-5218}\inst{\ref{aff149}}
\and A.~Calabro\orcid{0000-0003-2536-1614}\inst{\ref{aff22}}
\and B.~Camacho~Quevedo\orcid{0000-0002-8789-4232}\inst{\ref{aff37},\ref{aff40},\ref{aff38}}
\and F.~Caro\inst{\ref{aff22}}
\and C.~S.~Carvalho\inst{\ref{aff122}}
\and T.~Castro\orcid{0000-0002-6292-3228}\inst{\ref{aff38},\ref{aff39},\ref{aff37},\ref{aff138}}
\and F.~Cogato\orcid{0000-0003-4632-6113}\inst{\ref{aff93},\ref{aff4}}
\and S.~Conseil\orcid{0000-0002-3657-4191}\inst{\ref{aff29}}
\and A.~R.~Cooray\orcid{0000-0002-3892-0190}\inst{\ref{aff150}}
\and O.~Cucciati\orcid{0000-0002-9336-7551}\inst{\ref{aff4}}
\and G.~Daste\inst{\ref{aff62}}
\and F.~De~Paolis\orcid{0000-0001-6460-7563}\inst{\ref{aff134},\ref{aff135},\ref{aff136}}
\and G.~Desprez\orcid{0000-0001-8325-1742}\inst{\ref{aff2}}
\and A.~D\'iaz-S\'anchez\orcid{0000-0003-0748-4768}\inst{\ref{aff151}}
\and J.~J.~Diaz\orcid{0000-0003-2101-1078}\inst{\ref{aff58}}
\and S.~Di~Domizio\orcid{0000-0003-2863-5895}\inst{\ref{aff43},\ref{aff44}}
\and J.~M.~Diego\orcid{0000-0001-9065-3926}\inst{\ref{aff152}}
\and P.~Dimauro\orcid{0000-0001-7399-2854}\inst{\ref{aff153},\ref{aff22}}
\and P.-A.~Duc\orcid{0000-0003-3343-6284}\inst{\ref{aff146}}
\and M.~Y.~Elkhashab\orcid{0000-0001-9306-2603}\inst{\ref{aff38},\ref{aff39},\ref{aff148},\ref{aff37}}
\and A.~Enia\orcid{0000-0002-0200-2857}\inst{\ref{aff16},\ref{aff4}}
\and Y.~Fang\orcid{0000-0002-0334-6950}\inst{\ref{aff70}}
\and A.~G.~Ferrari\orcid{0009-0005-5266-4110}\inst{\ref{aff41}}
\and A.~Finoguenov\orcid{0000-0002-4606-5403}\inst{\ref{aff85}}
\and F.~Fontanot\orcid{0000-0003-4744-0188}\inst{\ref{aff38},\ref{aff37}}
\and A.~Franco\orcid{0000-0002-4761-366X}\inst{\ref{aff135},\ref{aff134},\ref{aff136}}
\and K.~Ganga\orcid{0000-0001-8159-8208}\inst{\ref{aff95}}
\and J.~Garc\'ia-Bellido\orcid{0000-0002-9370-8360}\inst{\ref{aff139}}
\and T.~Gasparetto\orcid{0000-0002-7913-4866}\inst{\ref{aff22}}
\and V.~Gautard\inst{\ref{aff154}}
\and E.~Gaztanaga\orcid{0000-0001-9632-0815}\inst{\ref{aff35},\ref{aff72},\ref{aff155}}
\and F.~Giacomini\orcid{0000-0002-3129-2814}\inst{\ref{aff41}}
\and F.~Gianotti\orcid{0000-0003-4666-119X}\inst{\ref{aff4}}
\and G.~Gozaliasl\orcid{0000-0002-0236-919X}\inst{\ref{aff156},\ref{aff85}}
\and M.~Gray\inst{\ref{aff62}}
\and M.~Guidi\orcid{0000-0001-9408-1101}\inst{\ref{aff16},\ref{aff4}}
\and C.~M.~Gutierrez\orcid{0000-0001-7854-783X}\inst{\ref{aff34}}
\and A.~Hall\orcid{0000-0002-3139-8651}\inst{\ref{aff33}}
\and C.~Hern\'andez-Monteagudo\orcid{0000-0001-5471-9166}\inst{\ref{aff113},\ref{aff58}}
\and H.~Hildebrandt\orcid{0000-0002-9814-3338}\inst{\ref{aff157}}
\and J.~Hjorth\orcid{0000-0002-4571-2306}\inst{\ref{aff104}}
\and J.~J.~E.~Kajava\orcid{0000-0002-3010-8333}\inst{\ref{aff158},\ref{aff159}}
\and Y.~Kang\orcid{0009-0000-8588-7250}\inst{\ref{aff14}}
\and V.~Kansal\orcid{0000-0002-4008-6078}\inst{\ref{aff160},\ref{aff161}}
\and D.~Karagiannis\orcid{0000-0002-4927-0816}\inst{\ref{aff125},\ref{aff162}}
\and K.~Kiiveri\inst{\ref{aff83}}
\and J.~Kim\orcid{0000-0003-2776-2761}\inst{\ref{aff130}}
\and C.~C.~Kirkpatrick\inst{\ref{aff83}}
\and S.~Kruk\orcid{0000-0001-8010-8879}\inst{\ref{aff61}}
\and V.~Le~Brun\orcid{0000-0002-5027-1939}\inst{\ref{aff62}}
\and J.~Le~Graet\orcid{0000-0001-6523-7971}\inst{\ref{aff69}}
\and L.~Legrand\orcid{0000-0003-0610-5252}\inst{\ref{aff163},\ref{aff164}}
\and M.~Lembo\orcid{0000-0002-5271-5070}\inst{\ref{aff99},\ref{aff125},\ref{aff126}}
\and F.~Lepori\orcid{0009-0000-5061-7138}\inst{\ref{aff165}}
\and G.~Leroy\orcid{0009-0004-2523-4425}\inst{\ref{aff23},\ref{aff94}}
\and G.~F.~Lesci\orcid{0000-0002-4607-2830}\inst{\ref{aff93},\ref{aff4}}
\and J.~Lesgourgues\orcid{0000-0001-7627-353X}\inst{\ref{aff53}}
\and T.~I.~Liaudat\orcid{0000-0002-9104-314X}\inst{\ref{aff145}}
\and A.~Loureiro\orcid{0000-0002-4371-0876}\inst{\ref{aff166},\ref{aff167}}
\and J.~Macias-Perez\orcid{0000-0002-5385-2763}\inst{\ref{aff168}}
\and M.~Magliocchetti\orcid{0000-0001-9158-4838}\inst{\ref{aff24}}
\and C.~Mancini\orcid{0000-0002-4297-0561}\inst{\ref{aff20}}
\and R.~Maoli\orcid{0000-0002-6065-3025}\inst{\ref{aff169},\ref{aff22}}
\and C.~J.~A.~P.~Martins\orcid{0000-0002-4886-9261}\inst{\ref{aff170},\ref{aff18}}
\and L.~Maurin\orcid{0000-0002-8406-0857}\inst{\ref{aff31}}
\and M.~Miluzio\inst{\ref{aff61},\ref{aff171}}
\and P.~Monaco\orcid{0000-0003-2083-7564}\inst{\ref{aff148},\ref{aff38},\ref{aff39},\ref{aff37},\ref{aff138}}
\and C.~Moretti\orcid{0000-0003-3314-8936}\inst{\ref{aff38},\ref{aff37},\ref{aff39},\ref{aff40}}
\and G.~Morgante\inst{\ref{aff4}}
\and S.~Nadathur\orcid{0000-0001-9070-3102}\inst{\ref{aff155}}
\and K.~Naidoo\orcid{0000-0002-9182-1802}\inst{\ref{aff155},\ref{aff82}}
\and P.~Natoli\orcid{0000-0003-0126-9100}\inst{\ref{aff125},\ref{aff126}}
\and A.~Navarro-Alsina\orcid{0000-0002-3173-2592}\inst{\ref{aff91}}
\and S.~Nesseris\orcid{0000-0002-0567-0324}\inst{\ref{aff139}}
\and D.~Paoletti\orcid{0000-0003-4761-6147}\inst{\ref{aff4},\ref{aff71}}
\and F.~Passalacqua\orcid{0000-0002-8606-4093}\inst{\ref{aff114},\ref{aff68}}
\and K.~Paterson\orcid{0000-0001-8340-3486}\inst{\ref{aff10}}
\and L.~Patrizii\inst{\ref{aff41}}
\and A.~Pisani\orcid{0000-0002-6146-4437}\inst{\ref{aff69}}
\and D.~Potter\orcid{0000-0002-0757-5195}\inst{\ref{aff165}}
\and S.~Quai\orcid{0000-0002-0449-8163}\inst{\ref{aff93},\ref{aff4}}
\and M.~Radovich\orcid{0000-0002-3585-866X}\inst{\ref{aff42}}
\and P.-F.~Rocci\inst{\ref{aff31}}
\and G.~Rodighiero\orcid{0000-0002-9415-2296}\inst{\ref{aff114},\ref{aff42}}
\and S.~Sacquegna\orcid{0000-0002-8433-6630}\inst{\ref{aff172},\ref{aff134},\ref{aff135}}
\and M.~Sahl\'en\orcid{0000-0003-0973-4804}\inst{\ref{aff173}}
\and D.~B.~Sanders\orcid{0000-0002-1233-9998}\inst{\ref{aff56}}
\and E.~Sarpa\orcid{0000-0002-1256-655X}\inst{\ref{aff40},\ref{aff138},\ref{aff39}}
\and C.~Scarlata\orcid{0000-0002-9136-8876}\inst{\ref{aff174}}
\and A.~Schneider\orcid{0000-0001-7055-8104}\inst{\ref{aff165}}
\and D.~Sciotti\orcid{0009-0008-4519-2620}\inst{\ref{aff22},\ref{aff92}}
\and E.~Sellentin\inst{\ref{aff175},\ref{aff1}}
\and F.~Shankar\orcid{0000-0001-8973-5051}\inst{\ref{aff9}}
\and L.~C.~Smith\orcid{0000-0002-3259-2771}\inst{\ref{aff176}}
\and E.~Soubrie\orcid{0000-0001-9295-1863}\inst{\ref{aff31}}
\and K.~Tanidis\orcid{0000-0001-9843-5130}\inst{\ref{aff130}}
\and C.~Tao\orcid{0000-0001-7961-8177}\inst{\ref{aff69}}
\and G.~Testera\inst{\ref{aff44}}
\and R.~Teyssier\orcid{0000-0001-7689-0933}\inst{\ref{aff177}}
\and S.~Tosi\orcid{0000-0002-7275-9193}\inst{\ref{aff43},\ref{aff44},\ref{aff36}}
\and A.~Troja\orcid{0000-0003-0239-4595}\inst{\ref{aff114},\ref{aff68}}
\and M.~Tucci\inst{\ref{aff14}}
\and C.~Valieri\inst{\ref{aff41}}
\and A.~Venhola\orcid{0000-0001-6071-4564}\inst{\ref{aff178}}
\and G.~Verza\orcid{0000-0002-1886-8348}\inst{\ref{aff179}}
\and P.~Vielzeuf\orcid{0000-0003-2035-9339}\inst{\ref{aff69}}
\and A.~Viitanen\orcid{0000-0001-9383-786X}\inst{\ref{aff83},\ref{aff14},\ref{aff22}}
\and N.~A.~Walton\orcid{0000-0003-3983-8778}\inst{\ref{aff176}}
\and J.~R.~Weaver\orcid{0000-0003-1614-196X}\inst{\ref{aff180},\ref{aff181}}}
										   
%%%% please do not edit the affiliation list -- contact ECEB Bureau for changes
\institute{Leiden Observatory, Leiden University, Einsteinweg 55, 2333 CC Leiden, The Netherlands\label{aff1}
\and
Kapteyn Astronomical Institute, University of Groningen, PO Box 800, 9700 AV Groningen, The Netherlands\label{aff2}
\and
Cosmic Dawn Center (DAWN)\label{aff3}
\and
INAF-Osservatorio di Astrofisica e Scienza dello Spazio di Bologna, Via Piero Gobetti 93/3, 40129 Bologna, Italy\label{aff4}
\and
Dipartimento di Fisica e Astronomia, Universit\`{a} di Firenze, via G. Sansone 1, 50019 Sesto Fiorentino, Firenze, Italy\label{aff5}
\and
University of Trento, Via Sommarive 14, I-38123 Trento, Italy\label{aff6}
\and
INAF-Osservatorio Astrofisico di Arcetri, Largo E. Fermi 5, 50125, Firenze, Italy\label{aff7}
\and
SRON Netherlands Institute for Space Research, Landleven 12, 9747 AD, Groningen, The Netherlands\label{aff8}
\and
School of Physics \& Astronomy, University of Southampton, Highfield Campus, Southampton SO17 1BJ, UK\label{aff9}
\and
Max-Planck-Institut f\"ur Astronomie, K\"onigstuhl 17, 69117 Heidelberg, Germany\label{aff10}
\and
Department of Physical Sciences, Ritsumeikan University, Kusatsu, Shiga 525-8577, Japan\label{aff11}
\and
Academia Sinica Institute of Astronomy and Astrophysics (ASIAA), 11F of ASMAB, No.~1, Section 4, Roosevelt Road, Taipei 10617, Taiwan\label{aff12}
\and
INAF-Osservatorio Astronomico di Capodimonte, Via Moiariello 16, 80131 Napoli, Italy\label{aff13}
\and
Department of Astronomy, University of Geneva, ch. d'Ecogia 16, 1290 Versoix, Switzerland\label{aff14}
\and
Institute for Particle Physics and Astrophysics, Dept. of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 27, 8093 Zurich, Switzerland\label{aff15}
\and
Dipartimento di Fisica e Astronomia, Universit\`a di Bologna, Via Gobetti 93/2, 40129 Bologna, Italy\label{aff16}
\and
Faculdade de Ci\^encias da Universidade do Porto, Rua do Campo de Alegre, 4150-007 Porto, Portugal\label{aff17}
\and
Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Universidade do Porto, CAUP, Rua das Estrelas, PT4150-762 Porto, Portugal\label{aff18}
\and
DTx -- Digital Transformation CoLAB, Building 1, Azur\'em Campus, University of Minho, 4800-058 Guimar\~aes, Portugal\label{aff19}
\and
INAF-IASF Milano, Via Alfonso Corti 12, 20133 Milano, Italy\label{aff20}
\and
Department of Mathematics and Physics, Roma Tre University, Via della Vasca Navale 84, 00146 Rome, Italy\label{aff21}
\and
INAF-Osservatorio Astronomico di Roma, Via Frascati 33, 00078 Monteporzio Catone, Italy\label{aff22}
\and
Department of Physics, Centre for Extragalactic Astronomy, Durham University, South Road, Durham, DH1 3LE, UK\label{aff23}
\and
INAF-Istituto di Astrofisica e Planetologia Spaziali, via del Fosso del Cavaliere, 100, 00100 Roma, Italy\label{aff24}
\and
School of Physics, HH Wills Physics Laboratory, University of Bristol, Tyndall Avenue, Bristol, BS8 1TL, UK\label{aff25}
\and
Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA, 91109, USA\label{aff26}
\and
Mullard Space Science Laboratory, University College London, Holmbury St Mary, Dorking, Surrey RH5 6NT, UK\label{aff27}
\and
Max Planck Institute for Extraterrestrial Physics, Giessenbachstr. 1, 85748 Garching, Germany\label{aff28}
\and
Universit\'e Claude Bernard Lyon 1, CNRS/IN2P3, IP2I Lyon, UMR 5822, Villeurbanne, F-69100, France\label{aff29}
\and
Univ. Lille, CNRS, Centrale Lille, UMR 9189 CRIStAL, 59000 Lille, France\label{aff30}
\and
Universit\'e Paris-Saclay, CNRS, Institut d'astrophysique spatiale, 91405, Orsay, France\label{aff31}
\and
Department of Physics and Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada\label{aff32}
\and
Institute for Astronomy, University of Edinburgh, Royal Observatory, Blackford Hill, Edinburgh EH9 3HJ, UK\label{aff33}
\and
 Instituto de Astrof\'{\i}sica de Canarias, E-38205 La Laguna; Universidad de La Laguna, Dpto. Astrof\'\i sica, E-38206 La Laguna, Tenerife, Spain\label{aff34}
\and
Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Can Magrans, s/n, 08193 Barcelona, Spain\label{aff35}
\and
INAF-Osservatorio Astronomico di Brera, Via Brera 28, 20122 Milano, Italy\label{aff36}
\and
IFPU, Institute for Fundamental Physics of the Universe, via Beirut 2, 34151 Trieste, Italy\label{aff37}
\and
INAF-Osservatorio Astronomico di Trieste, Via G. B. Tiepolo 11, 34143 Trieste, Italy\label{aff38}
\and
INFN, Sezione di Trieste, Via Valerio 2, 34127 Trieste TS, Italy\label{aff39}
\and
SISSA, International School for Advanced Studies, Via Bonomea 265, 34136 Trieste TS, Italy\label{aff40}
\and
INFN-Sezione di Bologna, Viale Berti Pichat 6/2, 40127 Bologna, Italy\label{aff41}
\and
INAF-Osservatorio Astronomico di Padova, Via dell'Osservatorio 5, 35122 Padova, Italy\label{aff42}
\and
Dipartimento di Fisica, Universit\`a di Genova, Via Dodecaneso 33, 16146, Genova, Italy\label{aff43}
\and
INFN-Sezione di Genova, Via Dodecaneso 33, 16146, Genova, Italy\label{aff44}
\and
Department of Physics "E. Pancini", University Federico II, Via Cinthia 6, 80126, Napoli, Italy\label{aff45}
\and
European Southern Observatory, Karl-Schwarzschild-Str.~2, 85748 Garching, Germany\label{aff46}
\and
Dipartimento di Fisica, Universit\`a degli Studi di Torino, Via P. Giuria 1, 10125 Torino, Italy\label{aff47}
\and
INFN-Sezione di Torino, Via P. Giuria 1, 10125 Torino, Italy\label{aff48}
\and
INAF-Osservatorio Astrofisico di Torino, Via Osservatorio 20, 10025 Pino Torinese (TO), Italy\label{aff49}
\and
European Space Agency/ESTEC, Keplerlaan 1, 2201 AZ Noordwijk, The Netherlands\label{aff50}
\and
Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Avenida Complutense 40, 28040 Madrid, Spain\label{aff51}
\and
Port d'Informaci\'{o} Cient\'{i}fica, Campus UAB, C. Albareda s/n, 08193 Bellaterra (Barcelona), Spain\label{aff52}
\and
Institute for Theoretical Particle Physics and Cosmology (TTK), RWTH Aachen University, 52056 Aachen, Germany\label{aff53}
\and
Deutsches Zentrum f\"ur Luft- und Raumfahrt e. V. (DLR), Linder H\"ohe, 51147 K\"oln, Germany\label{aff54}
\and
INFN section of Naples, Via Cinthia 6, 80126, Napoli, Italy\label{aff55}
\and
Institute for Astronomy, University of Hawaii, 2680 Woodlawn Drive, Honolulu, HI 96822, USA\label{aff56}
\and
Dipartimento di Fisica e Astronomia "Augusto Righi" - Alma Mater Studiorum Universit\`a di Bologna, Viale Berti Pichat 6/2, 40127 Bologna, Italy\label{aff57}
\and
Instituto de Astrof\'{\i}sica de Canarias, E-38205 La Laguna, Tenerife, Spain\label{aff58}
\and
Jodrell Bank Centre for Astrophysics, Department of Physics and Astronomy, University of Manchester, Oxford Road, Manchester M13 9PL, UK\label{aff59}
\and
European Space Agency/ESRIN, Largo Galileo Galilei 1, 00044 Frascati, Roma, Italy\label{aff60}
\and
ESAC/ESA, Camino Bajo del Castillo, s/n., Urb. Villafranca del Castillo, 28692 Villanueva de la Ca\~nada, Madrid, Spain\label{aff61}
\and
Aix-Marseille Universit\'e, CNRS, CNES, LAM, Marseille, France\label{aff62}
\and
Institut de Ci\`{e}ncies del Cosmos (ICCUB), Universitat de Barcelona (IEEC-UB), Mart\'{i} i Franqu\`{e}s 1, 08028 Barcelona, Spain\label{aff63}
\and
Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats (ICREA), Passeig de Llu\'{\i}s Companys 23, 08010 Barcelona, Spain\label{aff64}
\and
UCB Lyon 1, CNRS/IN2P3, IUF, IP2I Lyon, 4 rue Enrico Fermi, 69622 Villeurbanne, France\label{aff65}
\and
Departamento de F\'isica, Faculdade de Ci\^encias, Universidade de Lisboa, Edif\'icio C8, Campo Grande, PT1749-016 Lisboa, Portugal\label{aff66}
\and
Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Faculdade de Ci\^encias, Universidade de Lisboa, Campo Grande, 1749-016 Lisboa, Portugal\label{aff67}
\and
INFN-Padova, Via Marzolo 8, 35131 Padova, Italy\label{aff68}
\and
Aix-Marseille Universit\'e, CNRS/IN2P3, CPPM, Marseille, France\label{aff69}
\and
Universit\"ats-Sternwarte M\"unchen, Fakult\"at f\"ur Physik, Ludwig-Maximilians-Universit\"at M\"unchen, Scheinerstr.~1, 81679 M\"unchen, Germany\label{aff70}
\and
INFN-Bologna, Via Irnerio 46, 40126 Bologna, Italy\label{aff71}
\and
Institut d'Estudis Espacials de Catalunya (IEEC),  Edifici RDIT, Campus UPC, 08860 Castelldefels, Barcelona, Spain\label{aff72}
\and
University Observatory, LMU Faculty of Physics, Scheinerstr.~1, 81679 Munich, Germany\label{aff73}
\and
Dipartimento di Fisica "Aldo Pontremoli", Universit\`a degli Studi di Milano, Via Celoria 16, 20133 Milano, Italy\label{aff74}
\and
INFN-Sezione di Milano, Via Celoria 16, 20133 Milano, Italy\label{aff75}
\and
Institute of Theoretical Astrophysics, University of Oslo, P.O. Box 1029 Blindern, 0315 Oslo, Norway\label{aff76}
\and
Department of Physics, Lancaster University, Lancaster, LA1 4YB, UK\label{aff77}
\and
Felix Hormuth Engineering, Goethestr. 17, 69181 Leimen, Germany\label{aff78}
\and
Technical University of Denmark, Elektrovej 327, 2800 Kgs. Lyngby, Denmark\label{aff79}
\and
Cosmic Dawn Center (DAWN), Denmark\label{aff80}
\and
NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA\label{aff81}
\and
Department of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT, UK\label{aff82}
\and
Department of Physics and Helsinki Institute of Physics, Gustaf H\"allstr\"omin katu 2, University of Helsinki, 00014 Helsinki, Finland\label{aff83}
\and
Universit\'e de Gen\`eve, D\'epartement de Physique Th\'eorique and Centre for Astroparticle Physics, 24 quai Ernest-Ansermet, CH-1211 Gen\`eve 4, Switzerland\label{aff84}
\and
Department of Physics, P.O. Box 64, University of Helsinki, 00014 Helsinki, Finland\label{aff85}
\and
Helsinki Institute of Physics, Gustaf H{\"a}llstr{\"o}min katu 2, University of Helsinki, 00014 Helsinki, Finland\label{aff86}
\and
Laboratoire d'etude de l'Univers et des phenomenes eXtremes, Observatoire de Paris, Universit\'e PSL, Sorbonne Universit\'e, CNRS, 92190 Meudon, France\label{aff87}
\and
SKAO, Jodrell Bank, Lower Withington, Macclesfield SK11 9FT, UK\label{aff88}
\and
Centre de Calcul de l'IN2P3/CNRS, 21 avenue Pierre de Coubertin 69627 Villeurbanne Cedex, France\label{aff89}
\and
University of Applied Sciences and Arts of Northwestern Switzerland, School of Computer Science, 5210 Windisch, Switzerland\label{aff90}
\and
Universit\"at Bonn, Argelander-Institut f\"ur Astronomie, Auf dem H\"ugel 71, 53121 Bonn, Germany\label{aff91}
\and
INFN-Sezione di Roma, Piazzale Aldo Moro, 2 - c/o Dipartimento di Fisica, Edificio G. Marconi, 00185 Roma, Italy\label{aff92}
\and
Dipartimento di Fisica e Astronomia "Augusto Righi" - Alma Mater Studiorum Universit\`a di Bologna, via Piero Gobetti 93/2, 40129 Bologna, Italy\label{aff93}
\and
Department of Physics, Institute for Computational Cosmology, Durham University, South Road, Durham, DH1 3LE, UK\label{aff94}
\and
Universit\'e Paris Cit\'e, CNRS, Astroparticule et Cosmologie, 75013 Paris, France\label{aff95}
\and
CNRS-UCB International Research Laboratory, Centre Pierre Bin\'etruy, IRL2007, CPB-IN2P3, Berkeley, USA\label{aff96}
\and
University of Applied Sciences and Arts of Northwestern Switzerland, School of Engineering, 5210 Windisch, Switzerland\label{aff97}
\and
Institut d'Astrophysique de Paris, 98bis Boulevard Arago, 75014, Paris, France\label{aff98}
\and
Institut d'Astrophysique de Paris, UMR 7095, CNRS, and Sorbonne Universit\'e, 98 bis boulevard Arago, 75014 Paris, France\label{aff99}
\and
Institute of Physics, Laboratory of Astrophysics, Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland\label{aff100}
\and
Telespazio UK S.L. for European Space Agency (ESA), Camino bajo del Castillo, s/n, Urbanizacion Villafranca del Castillo, Villanueva de la Ca\~nada, 28692 Madrid, Spain\label{aff101}
\and
Institut de F\'{i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona), Spain\label{aff102}
\and
School of Mathematics and Physics, University of Surrey, Guildford, Surrey, GU2 7XH, UK\label{aff103}
\and
DARK, Niels Bohr Institute, University of Copenhagen, Jagtvej 155, 2200 Copenhagen, Denmark\label{aff104}
\and
Waterloo Centre for Astrophysics, University of Waterloo, Waterloo, Ontario N2L 3G1, Canada\label{aff105}
\and
Department of Physics and Astronomy, University of Waterloo, Waterloo, Ontario N2L 3G1, Canada\label{aff106}
\and
Perimeter Institute for Theoretical Physics, Waterloo, Ontario N2L 2Y5, Canada\label{aff107}
\and
Universit\'e Paris-Saclay, Universit\'e Paris Cit\'e, CEA, CNRS, AIM, 91191, Gif-sur-Yvette, France\label{aff108}
\and
Space Science Data Center, Italian Space Agency, via del Politecnico snc, 00133 Roma, Italy\label{aff109}
\and
Centre National d'Etudes Spatiales -- Centre spatial de Toulouse, 18 avenue Edouard Belin, 31401 Toulouse Cedex 9, France\label{aff110}
\and
Institute of Space Science, Str. Atomistilor, nr. 409 M\u{a}gurele, Ilfov, 077125, Romania\label{aff111}
\and
Consejo Superior de Investigaciones Cientificas, Calle Serrano 117, 28006 Madrid, Spain\label{aff112}
\and
Universidad de La Laguna, Dpto. Astrof\'\i sica, E-38206 La Laguna, Tenerife, Spain\label{aff113}
\and
Dipartimento di Fisica e Astronomia "G. Galilei", Universit\`a di Padova, Via Marzolo 8, 35131 Padova, Italy\label{aff114}
\and
Institut f\"ur Theoretische Physik, University of Heidelberg, Philosophenweg 16, 69120 Heidelberg, Germany\label{aff115}
\and
Institut de Recherche en Astrophysique et Plan\'etologie (IRAP), Universit\'e de Toulouse, CNRS, UPS, CNES, 14 Av. Edouard Belin, 31400 Toulouse, France\label{aff116}
\and
Universit\'e St Joseph; Faculty of Sciences, Beirut, Lebanon\label{aff117}
\and
Departamento de F\'isica, FCFM, Universidad de Chile, Blanco Encalada 2008, Santiago, Chile\label{aff118}
\and
Universit\"at Innsbruck, Institut f\"ur Astro- und Teilchenphysik, Technikerstr. 25/8, 6020 Innsbruck, Austria\label{aff119}
\and
Satlantis, University Science Park, Sede Bld 48940, Leioa-Bilbao, Spain\label{aff120}
\and
Infrared Processing and Analysis Center, California Institute of Technology, Pasadena, CA 91125, USA\label{aff121}
\and
Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Faculdade de Ci\^encias, Universidade de Lisboa, Tapada da Ajuda, 1349-018 Lisboa, Portugal\label{aff122}
\and
Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200 Copenhagen, Denmark\label{aff123}
\and
Universidad Polit\'ecnica de Cartagena, Departamento de Electr\'onica y Tecnolog\'ia de Computadoras,  Plaza del Hospital 1, 30202 Cartagena, Spain\label{aff124}
\and
Dipartimento di Fisica e Scienze della Terra, Universit\`a degli Studi di Ferrara, Via Giuseppe Saragat 1, 44122 Ferrara, Italy\label{aff125}
\and
Istituto Nazionale di Fisica Nucleare, Sezione di Ferrara, Via Giuseppe Saragat 1, 44122 Ferrara, Italy\label{aff126}
\and
INAF, Istituto di Radioastronomia, Via Piero Gobetti 101, 40129 Bologna, Italy\label{aff127}
\and
Astronomical Observatory of the Autonomous Region of the Aosta Valley (OAVdA), Loc. Lignan 39, I-11020, Nus (Aosta Valley), Italy\label{aff128}
\and
Universit\'e C\^{o}te d'Azur, Observatoire de la C\^{o}te d'Azur, CNRS, Laboratoire Lagrange, Bd de l'Observatoire, CS 34229, 06304 Nice cedex 4, France\label{aff129}
\and
Department of Physics, Oxford University, Keble Road, Oxford OX1 3RH, UK\label{aff130}
\and
Universit\'e PSL, Observatoire de Paris, Sorbonne Universit\'e, CNRS, LERMA, 75014, Paris, France\label{aff131}
\and
Universit\'e Paris-Cit\'e, 5 Rue Thomas Mann, 75013, Paris, France\label{aff132}
\and
Aurora Technology for European Space Agency (ESA), Camino bajo del Castillo, s/n, Urbanizacion Villafranca del Castillo, Villanueva de la Ca\~nada, 28692 Madrid, Spain\label{aff133}
\and
Department of Mathematics and Physics E. De Giorgi, University of Salento, Via per Arnesano, CP-I93, 73100, Lecce, Italy\label{aff134}
\and
INFN, Sezione di Lecce, Via per Arnesano, CP-193, 73100, Lecce, Italy\label{aff135}
\and
INAF-Sezione di Lecce, c/o Dipartimento Matematica e Fisica, Via per Arnesano, 73100, Lecce, Italy\label{aff136}
\and
ICL, Junia, Universit\'e Catholique de Lille, LITL, 59000 Lille, France\label{aff137}
\and
ICSC - Centro Nazionale di Ricerca in High Performance Computing, Big Data e Quantum Computing, Via Magnanelli 2, Bologna, Italy\label{aff138}
\and
Instituto de F\'isica Te\'orica UAM-CSIC, Campus de Cantoblanco, 28049 Madrid, Spain\label{aff139}
\and
CERCA/ISO, Department of Physics, Case Western Reserve University, 10900 Euclid Avenue, Cleveland, OH 44106, USA\label{aff140}
\and
Technical University of Munich, TUM School of Natural Sciences, Physics Department, James-Franck-Str.~1, 85748 Garching, Germany\label{aff141}
\and
Max-Planck-Institut f\"ur Astrophysik, Karl-Schwarzschild-Str.~1, 85748 Garching, Germany\label{aff142}
\and
Laboratoire Univers et Th\'eorie, Observatoire de Paris, Universit\'e PSL, Universit\'e Paris Cit\'e, CNRS, 92190 Meudon, France\label{aff143}
\and
Departamento de F{\'\i}sica Fundamental. Universidad de Salamanca. Plaza de la Merced s/n. 37008 Salamanca, Spain\label{aff144}
\and
IRFU, CEA, Universit\'e Paris-Saclay 91191 Gif-sur-Yvette Cedex, France\label{aff145}
\and
Universit\'e de Strasbourg, CNRS, Observatoire astronomique de Strasbourg, UMR 7550, 67000 Strasbourg, France\label{aff146}
\and
Center for Data-Driven Discovery, Kavli IPMU (WPI), UTIAS, The University of Tokyo, Kashiwa, Chiba 277-8583, Japan\label{aff147}
\and
Dipartimento di Fisica - Sezione di Astronomia, Universit\`a di Trieste, Via Tiepolo 11, 34131 Trieste, Italy\label{aff148}
\and
California Institute of Technology, 1200 E California Blvd, Pasadena, CA 91125, USA\label{aff149}
\and
Department of Physics \& Astronomy, University of California Irvine, Irvine CA 92697, USA\label{aff150}
\and
Departamento F\'isica Aplicada, Universidad Polit\'ecnica de Cartagena, Campus Muralla del Mar, 30202 Cartagena, Murcia, Spain\label{aff151}
\and
Instituto de F\'isica de Cantabria, Edificio Juan Jord\'a, Avenida de los Castros, 39005 Santander, Spain\label{aff152}
\and
Observatorio Nacional, Rua General Jose Cristino, 77-Bairro Imperial de Sao Cristovao, Rio de Janeiro, 20921-400, Brazil\label{aff153}
\and
CEA Saclay, DFR/IRFU, Service d'Astrophysique, Bat. 709, 91191 Gif-sur-Yvette, France\label{aff154}
\and
Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth PO1 3FX, UK\label{aff155}
\and
Department of Computer Science, Aalto University, PO Box 15400, Espoo, FI-00 076, Finland\label{aff156}
\and
Ruhr University Bochum, Faculty of Physics and Astronomy, Astronomical Institute (AIRUB), German Centre for Cosmological Lensing (GCCL), 44780 Bochum, Germany\label{aff157}
\and
Department of Physics and Astronomy, Vesilinnantie 5, University of Turku, 20014 Turku, Finland\label{aff158}
\and
Serco for European Space Agency (ESA), Camino bajo del Castillo, s/n, Urbanizacion Villafranca del Castillo, Villanueva de la Ca\~nada, 28692 Madrid, Spain\label{aff159}
\and
ARC Centre of Excellence for Dark Matter Particle Physics, Melbourne, Australia\label{aff160}
\and
Centre for Astrophysics \& Supercomputing, Swinburne University of Technology,  Hawthorn, Victoria 3122, Australia\label{aff161}
\and
Department of Physics and Astronomy, University of the Western Cape, Bellville, Cape Town, 7535, South Africa\label{aff162}
\and
DAMTP, Centre for Mathematical Sciences, Wilberforce Road, Cambridge CB3 0WA, UK\label{aff163}
\and
Kavli Institute for Cosmology Cambridge, Madingley Road, Cambridge, CB3 0HA, UK\label{aff164}
\and
Department of Astrophysics, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland\label{aff165}
\and
Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, Stockholm, SE-106 91, Sweden\label{aff166}
\and
Astrophysics Group, Blackett Laboratory, Imperial College London, London SW7 2AZ, UK\label{aff167}
\and
Univ. Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 53, Avenue des Martyrs, 38000, Grenoble, France\label{aff168}
\and
Dipartimento di Fisica, Sapienza Universit\`a di Roma, Piazzale Aldo Moro 2, 00185 Roma, Italy\label{aff169}
\and
Centro de Astrof\'{\i}sica da Universidade do Porto, Rua das Estrelas, 4150-762 Porto, Portugal\label{aff170}
\and
HE Space for European Space Agency (ESA), Camino bajo del Castillo, s/n, Urbanizacion Villafranca del Castillo, Villanueva de la Ca\~nada, 28692 Madrid, Spain\label{aff171}
\and
INAF - Osservatorio Astronomico d'Abruzzo, Via Maggini, 64100, Teramo, Italy\label{aff172}
\and
Theoretical astrophysics, Department of Physics and Astronomy, Uppsala University, Box 516, 751 37 Uppsala, Sweden\label{aff173}
\and
Minnesota Institute for Astrophysics, University of Minnesota, 116 Church St SE, Minneapolis, MN 55455, USA\label{aff174}
\and
Mathematical Institute, University of Leiden, Einsteinweg 55, 2333 CA Leiden, The Netherlands\label{aff175}
\and
Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\label{aff176}
\and
Department of Astrophysical Sciences, Peyton Hall, Princeton University, Princeton, NJ 08544, USA\label{aff177}
\and
Space physics and astronomy research unit, University of Oulu, Pentti Kaiteran katu 1, FI-90014 Oulu, Finland\label{aff178}
\and
Center for Computational Astrophysics, Flatiron Institute, 162 5th Avenue, 10010, New York, NY, USA\label{aff179}
\and
Department of Physics, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\label{aff180}
\and
MIT Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\label{aff181}}    
